Your Consent Is Worth 75 Euros A Year -- Measurement and Lawfulness of Cookie Paywalls

Most websites offer their content for free, though this gratuity often comes with a counterpart: personal data is collected to finance these websites by resorting, mostly, to tracking and thus targeted advertising. Cookie walls and paywalls, used to retrieve consent, recently generated interest from EU DPAs and seemed to have grown in popularity. However, they have been overlooked by scholars. We present in this paper 1) the results of an exploratory study conducted on 2800 Central European websites to measure the presence and practices of cookie paywalls, and 2) a framing of their lawfulness amidst the variety of legal decisions and guidelines.

==> Your Consent Is Worth 75 Euros A Year – Measurement and Lawfulness of Cookie Paywalls/temp.tex <==
\begin{table}[H]
\centering
\caption{Presence of Paywall Categories}
\label{table:presence}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{\textbf{Title}}                                                        \\ \hline
\textbf{\#} & \textbf{Header 1} & \textbf{Header 2} & \textbf{Header 3} & \textbf{Header 4} \\ \hline
1           & xx                & 1981562           & A                 & xx                \\ \hline
\rowcolor{yellow}
2           & xx                & 782012            & A                 & xx                \\ \hline
3           & xx                & 130780            & B                 & xx                \\ \hline
4           & xx                & 123090            & A                 & xx                \\ \hline
5           & xx                & 82204             & A                 & xx                \\ \hline
\end{tabular}
\end{table}

==> temp.tex <==
\begin{table}[H]
\centering
\caption{Presence of Paywall Categories}
\label{table:presence}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{\textbf{Title}}                                                        \\ \hline
\textbf{\#} & \textbf{Header 1} & \textbf{Header 2} & \textbf{Header 3} & \textbf{Header 4} \\ \hline
1           & xx                & 1981562           & A                 & xx                \\ \hline
\rowcolor{yellow}
2           & xx                & 782012            & A                 & xx                \\ \hline
3           & xx                & 130780            & B                 & xx                \\ \hline
4           & xx                & 123090            & A                 & xx                \\ \hline
5           & xx                & 82204             & A                 & xx                \\ \hline
\end{tabular}
\end{table}
